Immersive Learning Frameworks: A Systematic Literature Review

Contribution: This secondary study examines the literature on immersive learning frameworks and reviews their state of the art. Frameworks have been categorized according to their purpose. In addition, the elements that compose them were also categorized. Some gaps were identified and proposed as a research roadmap. Background: Immersive technologies for education have been used for some years. Despite this, there are few works that aim to support the development and use of virtual environments for immersive learning. Research Questions: This systematic review has the following main research question: What is the state of the art of immersive learning frameworks? In order to answer this question, secondary research questions were defined: 1) what definitions of immersive learning were adopted in primary studies? 2) what are the purposes of use by the frameworks? 3) what are the elements that compose the frameworks? 4) what are the methods used to validate the frameworks? Methodology: As per the systematic review guidelines, this study followed a rigorous and replicable process for collecting and analyzing data. From 1721 articles identified in the search engines, 15 were selected after the inclusion and exclusion criteria. Findings: Most frameworks are models that investigate the causal relationship between immersive learning factors that influence learning outcomes. Although this theoretical aspect is important for the advancement of research, the area still lacks more practical frameworks that address more technical details and support development, as well as the use of immersive virtual environments by teachers and instructors.

==> Sections/background.tex <==
\section{Background}\label{sec:back}
% this section aims to define the main terms used throughout this study
% - Milgran's continuum (VR, MR and XR)
% - immersive learning / immersive education
% - virtual environments
Considering the purpose of this review, this section aims to present the main concepts involved in immersive technologies, as well as exposing the State of XR Report in detail.

\subsection{VR, MR and XR}
Milgram and Kishino \cite{milgram1994taxonomy} defined the transition between reality and virtuality through a diagram known as Milgram's continuum, as shown in Fig.\ref{fig:milgrams-continuum}. At one end is the real environment and at the other the virtual environment, and in the range are Augmented Reality (AR) and Augmented Virtuality (AV). AR is the insertion of virtual elements into the real environment and AV, in turn, is the incorporation of real elements into the virtual environment. Both AR and AV are part of a larger reality called Mixed Reality (MR). Therefore, MR technology has the ability to mix elements from the real and virtual worlds. An umbrella term that encompasses the entire spectrum of continuous virtuality is called eXtended Reality (XR). One of the main features of XR is to immerse the user in a fully synthetic computer generated environment. Thus, due to the immersion characteristic, the literature addresses both the term XR and ``immersive' to the computational systems included in the Virtuality Continuum.

\begin{figure}[!t]
\centering
\includegraphics[width=3.25in]{Figures/Milgrams-continuum.png}
\caption{Virtuality continuum \cite{milgram1994taxonomy}.}
\label{fig:milgrams-continuum}
\end{figure}
\subsection{Immersive Technologies}
It refers to computer systems (hardware and software) that enable a more intuitive human-computer interface through devices and sensors that interact with up to the 5 human senses. The main devices are Head-Mounted Display (HMD), also known as a headset, and interaction devices. Google Cardboard\footnote{https://arvr.google.com/cardboard/}, Oculus Quest 2\footnote{https://www.oculus.com/quest-2/} and HTC Vive Pro 2\footnote{https: //www.vive.com/us/product/vive-pro2/overview/} are examples of VR headsets while Microsoft HoloLens 2\footnote{https://www.microsoft.com/en-us/hololens} is an example of MR headset. Generally, XR headsets, in addition to providing feedback through the visualization of 360º images and stereo audio, have controls for the hands in order to allow interaction with the virtual environment. Sensors that capture the movement of the hands (Leap Motion\footnote{https://www.ultraleap.com/product/leap-motion-controller/}) and the body (Omni One\footnote{https://invest.virtuix. com/}) can compose the virtual environment and enhance the immersive experience. Devices that allow you to experience the smell and taste, as well as feel the weight of virtual objects are still academic prototypes (see Section \ref{sec:level-imm}). Virtual environments, authoring tools and others are also part of XR systems.

\subsection{Virtual Environment (VE)}
Also known as a virtual world – it is a three-dimensional computer-generated space where users interact with each other (through avatars) or with other virtual objects \cite{biocca2013communication}. \citeauthor{sherman2003understanding} \cite{sherman2003understanding} define as the content of some medium. Virtual objects can manifest certain attributes, such as geometry, colors, textures, lighting, dynamic characteristics, physical constraints and \cite{fuchs2011virtual} acoustic attributes.

In some VEs, geometric precisions can be used, such as colors, textures and lighting, which are important elements to simulate the real world. However, certain VEs do not refer to the real world, constituting only abstract models. Regardless of the type of environment, colors, textures and lighting are important elements for good visualization and immersion. There are situations where the VE is used to evaluate only some behavioral simulation, in which the accuracy of the behavior is more important than the visual fidelity. This is the case for chemical reactions, which can use simple representations of molecules based on colored spheres, for example \cite{fuchs2011virtual}.

\subsection{Immersive Learning (iL)}
The definition of iL is one of the research questions of this secondary study. iL researchers have divergent understandings of trivial concepts such as immersion and presence, and this motivated us to obtain evidence from the literature regarding the understanding of iL. Considering our experience, we understand iL as an educational method that uses immersive technology as means to support the improvement of learning outcomes. This definition is similar to mobile learning (m-learning). The difference lies in the technological apparatus applied to teaching.

\subfile{state-xr-report}

==> Sections/introduction_v1.tex <==
\section{Introduction}

% popularização da VR com o metaverse
\IEEEPARstart{I}{n} October 2021, Facebook, now called Meta\footnote{https://about.fb.com/news/2021/10/facebook-company-is-now-meta/}, announced the plan to create the metaverse, a kind of universe in Augmented and Virtual Reality (AVR). After this announcement, the possibility of using immersive technologies for business, marketing, games and education became even more popular \cite{narin2021content}.

% benefícios das tecnologias imersivas na educação
Immersive technologies for education have been used for several years, mainly because virtual environments give the user the feeling of being present in the context that is presented, in addition to allowing the virtual manipulation of objects \cite{greenwald2017technology,fialho1999knowledge}. In situations where being physically present would be too expensive, dangerous or impossible, immersive experiences bring many advantages, for example in the training of surgical skills, pilots and astronauts \cite{fialho1999knowledge}. Furthermore, immersive experiences have greater engagement and allow greater interactivity of the student with the instructional material, encourages the collaborative construction of knowledge, presents more contextualized tasks, less abstract instructions and favors reflective practice \cite{bailenson2008use,lee2014learning}.

% desafios tecnologias imersivas na educação
Although virtual environments have already evolved a lot, there are still many research challenges involving immersive technologies in education \cite{RW18,RW49,ghinea2014mulsemedia}. In addition to the complexity of generating computational solutions for the specifics of educational demands, generally developed by researchers in the field of computing, there are challenges regarding pedagogical and psychological aspects, as well as user experience, storytelling, simulator sickness and others. In parallel, devices have evolved rapidly, allowing the use of virtual environments both in traditional devices (desktop and mobile) and in immersive devices (head-mounted display, motion sensors, and others). Despite the range of devices, developing for the various platforms is also challenging in order to ensure effective platform-independent performance. The State of XR Report \cite{stateofxrreport2021} summarizes the main challenges for the adoption of immersive technologies in education in 6 categories: access, affordability, inadequate XR teacher training programs, interoperability, lack of content and lack of infrastructure and tech support.

% desafios tecnologias imersivas na educação:
% - ponto de vista tecnológico, pedagógio e psicológio
% - citar frameworks como iniciativas de melhoria em immersive learning
In order to solve the challenges mentioned above and to contribute to the evolution of research related to immersive technologies in education, Immersive Learning (iL) Frameworks have been a strategy that researchers have found to define a basic conceptual framework to gather concepts and design a comprehensive understanding of a given phenomenon in the context of iL \cite{regoniel2015conceptual,jabareen2009building}. Therefore, considering the challenges of immersive technologies in education and frameworks as solutions to these problems, this systematic literature review aims to provide evidence on the state of the art of iL Frameworks. More precisely, we are interested in understanding what the purposes are, the elements that compose them and how the frameworks contribute to the solution of the main challenges, according to the State of XR Report \cite{stateofxrreport2021}, in addition to identifying gaps and opportunities for future research.
%Therefore, this systematic literature review aims to identify studies that support the use of immersive technologies in education. More precisely, the study aims to provide an overview of immersive learning frameworks as well as identifying gaps and opportunities for future research.

% seções do artigo
This article is organized as follows: Section \ref{sec:back} defines main concepts used throughout this work. Section \ref{sec:related} presents some previous secondary studies on Immersive Learning. Section \ref{sec:method} describes the research method and the article selection process. Section \ref{sec:results} presents the answers to the research questions. Section \ref{section:discussion} discusses the relevant findings, as well as a research roadmap and, finally, conclusions and future work are presented in Section \ref{sec:conclusion}.

\begin{comment}
No estudo de \textbf{Ashtari et al. (2020)}, aponta 8 principais barreiras para o desenvolvimento de conteúdos para ambientes virtuais. Dentre estas barreiras, destacam-se questões triviais da Engenharia de Software, tais como a falta de design guidelines; na escassez de estratégias viáveis no teste e depuparação de aplicações, bem como problemas relacionados avaliações e testes com usuários. 

O State of XR aponta que as principais barreiras para adoção de tecnologias imersivas na educação consiste que XR systems precisam evoluir em questões de acessibilidade; a aquisiação e manutenção de XR infrasctructures ainda é cara; programas e treinamentos de educadores são inadequados; há falta de padrões interoperáveis; há escassez de conteúdos educacionais e pouco suporte para garantir o desempenho do hardware, software e rede dos XR systems. 

Cerca de 100 educadores, pesquisadores e expecialistas contribuiram para State of XR \& Immersive Learning Outlook Report e apresentam um conjunto de oportunidades, tecnologias e principais barreiras em Immersve Learning. 

-------------------

% conceito de framework
% from: http://www.br-ie.org/pub/index.php/sbie/article/download/6829/4714
O termo framework adotado neste trabalho define uma estrutura conceitual básica de itens de ensino/aprendizagem aplicada no domínio de Engenharia de Software, sendo adaptável e reutilizável no contexto de disciplinas da graduação em Ciência da Computação, fornecendo apoio a professores e alunos.

% from: https://repositorio.ufpe.br/bitstream/123456789/37909/1/DISSERTAÇÃO%20Sandrine%20Ventura%20Martins.pdf
Um framework conceitual pode ser definido como uma estrutura usada para entender o contexto e informar a direção de um projeto de pesquisa, usando suas informações para orientar o planejamento deste projeto (MAGHER, 2016).
Frameworks conceituais são produtos gerados de processos qualitativos que reúnem conceitos para fornecer a compreensão abrangente de um fenômeno (JABA-REEN, 2009).
\end{comment}

==> Sections/state-xr-report.tex <==
\subsection{State of XR Report}
The State of XR Report \cite{stateofxrreport2021} is a body of knowledge based on research-based evidence on “what works” in iL. Organized by the Immersive Learning Research Network (iLRN), a nonprofit organization that connects researchers and educators, the report was developed through a rigorous several-month-long process with input from 100 experts from around the globe and representing diverse areas of education, industry and government all of whom are recognized for their leading-edge research, innovative practice within the field of XR and iL.

Approximately, 100 educators, researchers, technologists, and others representing diverse learning sectors were selected to join a global panel of experts. Each contributed with their perspectives on emerging and current trends, as well as important research and developments on the use of XR for supporting learning. As a result, the report groups the findings of the XR and iL study into three dimensions: the most important needs and opportunities, barriers to adoption, and catalyzing technologies and developments. In opportunities the advantages and in which areas XR has been and can be applied to support teaching and training are presented. Catalyst reports a set of technologies (Artificial Intelligence, Machine Learning, Games, Motion-caputre solutions and others) that has the potential to improve experiences during learning. According to the report's methodology, experts grouped the main barriers to adoption into: access, affordability, inadequate XR teacher training programs, interoperability, lack of content and lack of Infrastructure and tech support. Given our focus on mapping between frameworks and barriers to adoption, each challenge is detailed below.

\subsubsection{Access (B1)}
Access addresses issues related to limiting the distribution of immersive technologies, such as XR headsets, among countries that have world economic policies that hinder the commercialization of products. In addition, it considers an important aspect in the inclusion of people, which is the improvement of technologies and applications for people with disabilities. Most applications are visual and they still need more attention to solve this problem.

\subsubsection{Affordability (B2)}
From the affordability point of view, immersive experiences require equipment with high processing power for graphic rendering, in addition to specific equipment, such as XR headsets, motion sensors, among others. Therefore, economic availability is still a challenge for the implementation of immersive technologies, since the equipment has a high cost.

\subsubsection{Inadequate XR Teacher Training Programs (B3)}
For some institutions and professors, it is still a challenge to add immersive experiences to teaching practices, from a support point of view. XR headsets involve new ways of interaction between immersive application and device. Unlike the traditional keyboard, mouse and monitor, people need to gradually adapt to immersive applications. Additionally, immersive content must adhere to instructional purposes. Unfortunately, both technological and pedagogical support from educational institutions and some applications are incipient or non-existent. Educators need training programs on topics related to immersive technologies as well as instructional design support to successfully integrate XR into teaching practices.

\subsubsection{Interoperability (B4)}
Another challenge pointed out by experts is in relation to interoperability. Much immersive content is still locked into certain hardware, software and commercial frameworks. For educators, this presents a number of challenges, including difficulty adjusting specific technological resources to good pedagogical practices and longer training time across multiple platforms. For example, when choosing an XR headset, the equipment sets up a trajectory of subsequent decisions dependent on the implications of the device. Supporting user training, user requirements, and community ecosystems for each XR headset creates an effective environment for educators within which they are then limited, even though the same device can provide many benefits for education.

\subsubsection{Lack of Content (B5)}
As with all emerging technology, educators face the challenge of finding immersive instructional content or reusable content to leverage for educational use. A possible reason for this scenario is the amount of resources needed to develop immersive applications. Starting with the interdisciplinary development team that requires specialists with technical skills (software and sound engineers, game designers, 3D modelers), subject knowledge and audience understanding. These last two can be performed by educators, however, the technical aspect is certainly a challenge. Some tools have emerged to facilitate the creation of immersive content. However, for immersive applications to specifically address instructional content, authorial tools will require more technical knowledge from educators.

\subsubsection{Lack of Infrastructure and Tech Support (B6)}
Finally, the report presents the challenge of deploying an infrastructure of immersive systems. In addition to considering the challenge of cost-effective device availability, immersive applications depend on the integration between hardware, software and network in order to meet educational purposes. For example, work at schools from low socioeconomic and rural communities requires systems that adapt to mobile devices and available network bandwidth. Ensuring access to immersive experiences considering the available infrastructure and the audience context is still a challenge for iL.
